Robustness and Generalizability of Deepfake Detection: A Study with Diffusion Models

The rise of deepfake images, especially of well-known personalities, poses a serious threat to the dissemination of authentic information. To tackle this, we present a thorough investigation into how deepfakes are produced and how they can be identified. The cornerstone of our research is a rich collection of artificial celebrity faces, titled DeepFakeFace (DFF). We crafted the DFF dataset using advanced diffusion models and have shared it with the community through online platforms. This data serves as a robust foundation to train and test algorithms designed to spot deepfakes. We carried out a thorough review of the DFF dataset and suggest two evaluation methods to gauge the strength and adaptability of deepfake recognition tools. The first method tests whether an algorithm trained on one type of fake images can recognize those produced by other methods. The second evaluates the algorithm's performance with imperfect images, like those that are blurry, of low quality, or compressed. Given varied results across deepfake methods and image changes, our findings stress the need for better deepfake detectors. Our DFF dataset and tests aim to boost the development of more effective tools against deepfakes.

==> content/2_bak.tex <==
\section{Related Works}
This section offers an overview of prevailing deepfake detection datasets and methodologies. 

\subsection{Deepfake Generation}
% This is for related work.

% With the development of synthetic generation and  manipulation methods, deepfakes potentially pose a security concern since they might be exploited for nefarious bioinformatics purposes~\cite{arjovsky2017wasserstein,karras2019style,goodfellow2020generative}. 
In order to evaluate the effectiveness of various detection methods, many deefake datasets are proposed.
% ff++
Faceforensics++~\cite{rossler2019faceforensics++} is the most widely used dataset to assess the ability of detection methods. There are four kinds of manipulation methods: Deepfakes~\cite{deepfakes}, FaceSwap~\cite{faceswap}, Face2Face~\cite{thies2016face2face}, NeuralTextures~\cite{thies2019deferred}. Deepfakes~\cite{deepfakes} and FaceSwap~\cite{faceswap} exchange the identity of source image and target image, while Face2Face~\cite{thies2016face2face} and NeuralTextures~\cite{thies2019deferred} manipulate facial expression, maintaining the identity. FF++ dataset also provide three compression levels, raw, c23(high quality) and c40(low quality) to evaluate detection methods while facing compression situations. Due to the fact that the quality of some datasets is poor, Celeb-DF~\cite{li2020celeb} proposes an algorithm to achieve higher visual quality. There are 590 real videos and 5639 synthesized videos of celebrities in Celeb-DF dataset. In order to detect the manipulated faces in the real world, WildDeepfake~\cite{zi2020wilddeepfake} extracts 7314 sequences from 707 deepfake videos from the internet. DeepFake Detection Challenge Dataset (DFDC)~\cite{dolhansky2020deepfake} released by Google contains over 100,000 total clips. DFDC applies mulitiple methods such as Deepfake, GAN-based, and non-learned methods. However, such datasets synthesize deepfakes by swapping the faces of source and target images which may leave obvious boundaries. Thanks to the progress of generation technologies such as diffusion model, there are more and more deepfakes without stitching information. The GenImage dataset~\cite{zhu2023genimage} has significantly advanced deepfake detection by providing a large-scale dataset of AI-generated images. Our work, while aligned with GenImage in some aspects, distinguishes itself by specifically targeting synthetic faces of celebrities. Additionally, we introduce novel evaluation tasks, namely cross-generator image classification and degraded image classification, further enriching the evaluation of detection algorithm performance.

\input{tables/dataset_compare}

\subsection{Deepfake Detection}

% spatial-based

%Face X-ray for More General Face Forgery Detection
Face x-ray~\cite{li2020face} which is famous for its generalizability discriminate deepfakes by predicting if the input image contains blending boundaries. Instead of blending images with different identities, Shiohara \textit{et al.}\cite{shiohara2022detecting} blend images with the same identity.
% Face forgery Detection by 3D decomposition
Zhu~\cite{zhu2021face} first introduce 3D decomposition into deepfake detection and propose FD2Net to fuse the clues from input images and extracted facial details.
% Protecting Celebrities from DeepFake with Identity Consistency Transformer
Identity Consistency Transformer (ICT)~\cite{dong2022protecting} leverages  the freely available videos on the internet and measures the consistency of inner face and outer face regions.
%Multi-attentional Deepfake Detection
Zhao \textit{et al.}~\cite{zhao2021multi} views deepfake detection from a novel perspective, regarding deepfake detection as a fine-grained classification problem. To capture local features from various regions, they propose a new multi-attentional architecture network.
%Learning Self-Consistency for Deepfake Detection
Zhao \textit{et al.}~\cite{zhao2021learning} detect fogeries by measuring the consistencies of image patches.
%End-to-End Reconstruction-Classification Learning for Face Forgery Detection
RECCE~\cite{cao2022end} mines common features by only reconstructing genuine faces to distinguish real images from fake images.
%frequency(3 sentences)
Besides, researchers detect deepfakes by leveraging frequency clues~\cite{qian2020thinking,liu2021spatial,luo2021generalizing,li2021frequency}. 
%Thinking in Frequency: Face Forgery Detection by Mining Frequency-aware Clues
Qian \textit{et al.}~\cite{qian2020thinking} capture anomaly by frequency-aware decomposition and local frequency statistics. 
%Spatial-Phase Shallow Learning: Rethinking Face Forgery Detection in Frequency Domain
Spatial-Phase Shallow Learning method~\cite{liu2021spatial} leverage spatial image and phase spectrum simultaneously.
%Generalizing Face Forgery Detection with High-frequency Features
Luo \textit{et al.}~\cite{luo2021generalizing} capture the forgery through high-frequency noises.
There are also many methods detecting deefakes by introducing temporal information or auditory modality~\cite{zhou2021joint,haliassos2021lips,masi2020two,sun2021improving,zheng2021exploring,cozzolino2021id}.
% Lips don't lie: A generalisable and robust approach to face forgery detection
Haliassos \textit{et al.}~\cite{haliassos2021lips} leverage pretrained lip reading models to judge if the cropped mouth regions are from a real video.
% Joint audio-visual deepfake detection
Zhou \textit{et al.}~\cite{zhou2021joint} propose a sync-stream which detects whether the visual or auditory modality is manipulated. 
To evaluate the quality of our proposed dataset, we decide to adopt current state-of-the-art method, RECCE~\cite{cao2022end} which shows great superiority on cross-generator image classification and degraded image classification.


==> content/3_bak.tex <==
\section{Methodology}

This is for methodology.

\subsection{Dataset Details}
% To enable a precise assessment of a detector's ability to distinguish between AI-generated and authentic images, we curated a dataset named GenImage, comprising over one million pairs of real and fake images. GenImage is designed to align with the remarkable ImageNet dataset, encompassing all the real images from ImageNet. To ensure a balanced representation, the image generation process in GenImage leverages 1000 distinct labels from ImageNet, guaranteeing a nearly equal distribution of real and generated images across each class. The dataset consists of 2,681,167 images, divided into 1,331,167 real images and 1,350,000 fake images. Specifically, the real images are further categorized into 1,281,167 images for training and 50,000 images for testing.
% With ImageNet providing 1000 distinct image classes, we generated 1350 images for each class in GenImage. Out of these, 1300 images were allocated for training purposes, while the remaining 50 images were reserved for testing. To address the challenge of detecting images generated by state-of-the-art (SOTA) generators, we employed eight different generative models for image generation: BigGAN, GLIDE, VQDM, Stable Diffusion V1.4, Stable Diffusion V1.5, ADM, Midjourney, and Wukong. Each generator produced a nearly equal number of images for each class, with 162 images for training and 6 for testing, except for Stable Diffusion V1.5, which generated 166 training images and 8 testing images.
% To ensure a comprehensive exploration of each generator's properties when developing detection models, a combination of the generated fake images and their corresponding real images were considered as subsets (e.g., Stable Diffusion V1.4 subset). Importantly, the real images were not shared across subsets. The number of generated images approximated the number of real images for both the entire dataset and each subset, maintaining a balance that mitigates the impact of imbalances on the detection process.
% Our model input sentences followed the template "photo of class," with "class" being substituted by ImageNet labels. For Wukong, Chinese sentences were found to yield better generation quality, so the sentences were translated into Chinese for use with the web API. For ADM and BIGGAN, we utilized their pre-trained models on ImageNet, inputting the labels to generate images. The generated images can be viewed in Figure 1, and additional visualized images are available in the supplementary materials.
% Upon observation, it is evident that the generated images in GenImage exhibit an overall similarity to the real images in ImageNet. Instances of animals and plants successfully maintain the appearance of the target object, with similarities in features like a samoyed's appearance. However, they may differ in aspects such as movement, perspective, and background. For other objects like candles and lighthouses, the appearance of the targets varies to a certain degree. Consequently, the generated images demonstrate a high degree of variability and reasonableness."
We present a new dataset named DeepFakeFace (DFF) to assess the ability of deepfake detectors to distinguish AI-generated and authentic images. There are XX pairs of real and fake images. Since we aim to protect the privacy of celebrities, real images of XX dataset all comes from IMDB-WIKI dataset~\cite{rothe2015dex}. The dataset consists of XXX images which incorporate XX real images and XX fake images. Specifically, the real images are further categorized into XX images for training and XX images for testing. We employ three different generative models for synthesizing deepfakes: Stable Diffusion V1.5, Stable Diffusion Inpainting and XX. Each model generate XX images with XX images for training and XX images for testing.



\subsection{Fake Image Generators}
Diffusion models~\cite{ho2020denoising} synthesize high-resulution images by a sequential application of denoising autoencoders. However, directly operating on pixel space brings a high consumption on time and resources. Therefore, stable diffusion~\cite{rombach2022high} applies diffusion models in the latent space in order to reduce computational resources while retaining the quality and flexibility. Stable diffusion is capable of generating photo-realistic images given arbitrary input text. Hence, we utilize stable diffusion for generating fake images. The resolution of images generated by stable diffusion is 512 × 512. We adopt Stable Diffusion V1.5 and Stable Diffusion Inpainting models respectively. Stable Diffusion V1.5 is pretrained on Stable Diffusion V1.2 and fine-tune on 595k steps at resolution 512x512 on Laion-Aesthetics V2 5+ dataset and drops 10\% of the text-conditioning. Stable Diffusion Inpainting is also initialized with the weights of the Stable Diffusion V1.2. After regular training, Stable diffusion Inpainting fine tune on  440k steps. For inpainting, the UNet has 4 additional input channels for the encoded masked-image and 1 additional channel for the mask itself. Besides diffusion models, we also leverage a powerful toolbox insightface to generate deepfakes. InsightFace is an integrated Python library for 2D\&3D face analysis. There exists 
a rich variety of state of the art algorithms of face recognition, face detection ,face alignment and face swap algorithms. 

\subsection{Fake Image Generation process}
Since Imdb-WIKI dataset is the largest publicly available dataset of face images with gender and age labels for training, we can easily extract gender and age information from label file. Then, we randomly pair the images based on gender and all subsequent methods used follow this setting. After obtaining gender, age and the identity of each image, we generate prompts aligned with each image. Our input prompt follows the template "name, celebrity, age.", with "name" and being substituted by the identity and physical age of image. Although IMDB-WIKI dataset provides us the alighed faces and original facial bounding box, we find that some bounding boxes are not accurate. Therefore, we exploit state-of-the-art face detector RetianFace~\cite{deng2020retinaface} to generate facial bounding box and corresponding mask images. After preparing all the data, we leverage insightface, Stable Diffusion V1.5 and Stable Diffusion Inpainting to generate deepfake respectively.

==> figures/split_figure_example.tex <==
\begin{figure}[h]
\begin{center}
\subfloat[figure1]{\begin{centering}
\includegraphics[width=0.45\linewidth]{example-image-a}
\end{centering}
}\subfloat[figure2]{\begin{centering}
\includegraphics[width=0.45\linewidth]{example-image-b}
\end{centering}
}
\end{center}

\caption{(a) The first figure xxxx. 
(b)The second figure xxxxx.
}
\label{fig: split example}
\end{figure}

==> figures/wrapper_figure_example.tex <==
\begin{wrapfigure}{r}{8.5cm}
  \centering
  \includegraphics[width=0.95\linewidth]{example-image}
  \caption{Wrap figure example.
  }
  \label{fig:wrap figure example}
\end{wrapfigure}
